Homology computations for complex braid groups

Complex braid groups are the natural generalizations of braid groups associated to arbitrary (finite) complex reflection groups. We investigate several methods for computing the homology of these groups. In particular, we get the Poincar\'e polynomial with coefficients in a finite field for one large series of such groups, and compute the second integral cohomology group for all of them. As a consequence we get non-isomorphism results for these groups.

==> commands.tex <==
%\def\MR#1{\href{http://www.ams.org/mathscinet-getitem?mr=#1}{MR#1}}
%\def\MR#1{} 
%\def\MRhref#1{} 
\def\arxiv#1#2{\href{http://arxiv.org/abs/#1}{\texttt{arXiv:#1[math:#2]}}}
%%% Blackboard fonts

%\newcommand{\Z}[0]{\mathbb{Z}}
%\newcommand{\R}[0]{\mathbb{R}}
%\newcommand{\F}[0]{\mathbb{F}}
%\newcommand{\C}[0]{\mathbb{C}}
%\newcommand{\Q}[0]{\mathbb{Q}}
%\newcommand{\N}[0]{\mathbb{N}}
%\newcommand{\K}[0]{\mathbb{K}}
%\newcommand{\K}[0]{{K}}


\newcommand{\bd}[1]{\textbf{#1}} 			%grossetto
\newcommand{\mb}[1]{\mathbf{#1}}			%grossettoM
\newcommand{\q}[1]{\mbox{\bfseries{\textit{#1}}}} 
\newcommand{\itl}[1]{\textit{#1}} 			%corsivo
\newcommand{\g}[1]{\mathfrak{#1}} 			%goticoM
\newcommand{\geets}[0]{\longleftarrow}
\newcommand{\sst}[0]{\subset}
\newcommand{\cl}[1]{\mathcal{#1}}			%calligrafico
%\newcommand{\G}[0]{\mathcal{G}}
%\newcommand{\into}[0]{\hookrightarrow}
\newcommand{\codim}[0]{\mbox{codim }}
\newcommand{\diag}[0]{\Sigma}
\newcommand{\im}[0]{\mbox{im }}
\newcommand{\az}[0]{\"{a}}

%\newcommand{\n}[0]{ \{ n \} }
\renewcommand{\ni}[0]{\noindent}
\newcommand{\wI}[0]{\widetilde{I}}
\newcommand{\wqbin}[2]{ \widetilde{\left[ \begin{array}{c} #1 \\ #2 \end{array} \right] }}
\newcommand{\tss}[0]{\supset}
\newcommand{\CA}[0]{\overline{C}}
\newcommand{\modph}[0]{\hspace{1cm}\mbox{mod } \ph}
\newcommand{\lar}[1]{\stackrel{#1}{\leftarrow}}		%leftarrow

\newcommand{\pr}{\mathrm{Prod}}
\newcommand{\p}[0]{p}
\newcommand{\api}[0]{\p^{i-1}}
\newcommand{\bpi}[0]{\phi(p^i)}
\renewcommand{\cong}{\simeq}
%\renewcommand{\i}{{\mathrm{i}}}
\newcommand{\oC}[0]{L^1}
\newcommand{\cF}[0]{\mathcal{F}}
\renewcommand{\S}[0]{\mathfrak{S}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A refined command for quod erat demonstrandum %
\def\qed{\ifmmode $\Box$ \else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil $\Box$
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% per poincare' series ....poi si vedra'!           %
%\def\W{\mathbb W}
\def\W{W}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{plain}
\newtheorem{teo}{Theorem}[section]
\newtheorem*{teo*}{Theorem}
\newtheorem{lem}[teo]{Lemma}
%\newtheorem{cor}[teo]{Corollary}
%\newtheorem{prop}[teo]{Proposition}

\theoremstyle{definition}
\newtheorem{df}[teo]{Definition}
\newtheorem{es}[teo]{Example}
%\newtheorem{xca}[teo]{Exercise}

\theoremstyle{remark}
\newtheorem{os}[teo]{Remark}

\newenvironment{dm}[0]{\begin{proof}[Proof.]}{\end{proof}}
%\newenvironment{dm}[1][Proof.]{\begin{trivlist} \item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\numberwithin{equation}{section}


%%%%%%%%%%% Strings ///Filippo
\newcommand{\fbin}[2]{ \left\{ \begin{array}{c} #1 \\ #2  \end{array}  \right\} }
\newcommand{{\abin}}[2]{  \begin{array}{c} #1 \\ #2 \end{array}  }

%%%%%%%%%%%%%%%%%%

\newcommand{\re}{{\mathbf{R}}}
%\newcommand{\A}{{\mathcal{A}}}
%\newcommand{\B}{{\mathcal{B}}}
\newcommand{\cL}{{\mathcal{L}}}


\newcommand{\X}{{\mb{X}}}
\newcommand{\Y}{{\mb{Y}}}
\newcommand{\bQ}{{\mb{Q}}}
%\newcommand{\F}{{\mb{F}}}
\newcommand{\cs}{{\mb{C}}}
\newcommand{\M}{{\mb{M}}}
\renewcommand{\H}{{\mb{H}}}
\newcommand{\V}{{\mb{V}}}
\newcommand{\E}{{\mb{E}}}
\newcommand{\GL}{{\mb{GL}}}
\newcommand{\zZ}{{\mb{Z}}}
\newcommand{\G}{{\mb{G}}}


\providecommand{\A}{{\mathbf{A}}}
\providecommand{\q}{{\mathbf{q}}}
\newcommand{\lie}[2]{{[ #1 , #2  ]}}
\newcommand{\bra}[2]{{\langle #1, #2 \rangle}}
\newcommand{\no}[1]{{| #1 |}}
\newcommand{\inv}{I}
\newcommand{\anti}{K}

\newcommand{\imm}[1][r] {\ar@{^{(}->}[#1]}
\newcommand{\eq}[1][r]
       {\ar@<-3pt>@{-}[#1]
        \ar@<-1pt>@{}[#1]|<{}="gauche"
        \ar@<+0pt>@{}[#1]|-{}="milieu"
        \ar@<+1pt>@{}[#1]|>{}="droite"
        \ar@/^2pt/@{-}"gauche";"milieu"
        \ar@/_2pt/@{-}"milieu";"droite"}

\newcommand{\til}[1]{\widetilde{#1}}

\renewcommand{\t}[1]{\tilde{#1}}		
\newcommand{\qa}[1]{[#1]}		
\newcommand{\card}[1]{|#1|}
\newcommand{\de}{\partial}
\renewcommand{\mod}[1]{\,\mathrm{mod}(#1)}
\newcommand{\ch}{\mathrm{char}}
%%newcommand{\char}{\mathrm{char}}
\newcommand{\Id}{\mathrm{Id}}


%\newcommand*\bigdot{${\mathbin{\raise.29ex\hbox{$\scriptscriptstyle{\bullet}$}}}$}

%come andrebbero definiti gli operatori matematici
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Tor}{Tor}
\renewcommand{\l}{\mathrm{l}}
%\newcommand{\ker}{\mathrm{ker}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\Aff}{\mathrm{Aff}}
\newcommand{\ind}{\mathrm{Ind}}
\newcommand{\coind}{\mathrm{CoInd}}
\newcommand{\Aut}{\mathrm{Aut}}
%Bordo di cocatene
\newcommand{\di}{{\mathrm{d}}}
\newcommand{\res}{{\mathrm{res}}}



